Illuminating the Space of Enemies Through MAP-Elites

Action-Adventure games have several challenges to overcome, where the most common are enemies. The enemies' goal is to hinder the players' progression by taking life points, and the way they hinder this progress is distinct for different kinds of enemies. In this context, this paper introduces an extended version of an evolutionary approach for procedurally generating enemies that target the enemy's difficulty as the goal. Our approach advances the enemy generation research by incorporating a MAP-Elites population to generate diverse enemies without losing quality. The computational experiment showed the method converged most enemies in the MAP-Elites in less than a second for most cases. Besides, we experimented with players who played an Action-Adventure game prototype with enemies we generated. This experiment showed that the players enjoyed most levels they played, and we successfully created enemies perceived as easy, medium, or hard to face.

==> Breno CoG2022/images/enemies.tex <==
\begin{figure}[!t]
\centering

    \begin{subfigure}[t]{.15\textwidth}
    \centering
    \includegraphics[width=.35\linewidth]{images/enemies/Slime.png}
    \subcaption{Slime (no weapon).}
    \label{fig:e1}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.15\textwidth}
    \centering
    \includegraphics[width=.5\linewidth]{images/enemies/EnemySword.png}
    \subcaption{Swordsman.}
    \label{fig:e2}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.15\textwidth}
    \centering
    \includegraphics[width=.3\linewidth]{images/enemies/RedMage.png}
    \subcaption{Bower mage.}
    \label{fig:e3}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.15\textwidth}
    \centering
    \includegraphics[width=.3\linewidth]{images/enemies/GreenMage.png}
    \subcaption{Bomber mage.}
    \label{fig:e4}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.15\textwidth}
    \centering
    \includegraphics[width=.5\linewidth]{images/enemies/EnemyShield.png}
    \subcaption{Shieldsman.}
    \label{fig:e5}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{.15\textwidth}
    \centering
    \includegraphics[width=.3\linewidth]{images/enemies/BlueMage.png}
    \subcaption{Healer (Cure Spell).}
    \label{fig:e6}
    \end{subfigure}


\caption{List of enemies of our game prototype. Slimes have no weapon. Swordsmans use swords. Bower mages shoot arrows. Bomber mages throw bombs. Shieldsmans hold shields. Healers use cure spell to heal other enemies.}
\label{fig:enemies}

\end{figure}

==> Breno CoG2022/images/methodology/map-representation.tex <==
\begin{figure}[!t]
    \centering
    \begin{tikzpicture}[every node/.style={scale=0.6}]
    % Node style
    \tikzstyle{node} = [draw, minimum size=1cm]

    % 
    \node[node] (l1c1) at (0,0) { };
    \node[node] (l1c2) [right = 0.5cm of l1c1] { };
    \node[node] (l1c3) [right = 0.5cm of l1c2] { };
    \node[node] (l1c4) [right = 0.5cm of l1c3] { };
    \node[node] (l1c5) [right = 0.5cm of l1c4] { };
    \node[node] (l1c6) [right = 0.5cm of l1c5] { };
    % 
    \node[node] (l2c1) [below = 0.1cm of l1c1] { };
    \node[node] (l2c2) [right = 0.5cm of l2c1] { };
    \node[node] (l2c3) [right = 0.5cm of l2c2] { };
    \node[node] (l2c4) [right = 0.5cm of l2c3] { };
    \node[node] (l2c5) [right = 0.5cm of l2c4] { };
    \node[node] (l2c6) [right = 0.5cm of l2c5] { };
    % 
    \node[node] (l3c1) [below = 0.1cm of l2c1] { };
    \node[node] (l3c2) [right = 0.5cm of l3c1] { };
    \node[node] (l3c3) [right = 0.5cm of l3c2] { };
    \node[node] (l3c4) [right = 0.5cm of l3c3] { };
    \node[node] (l3c5) [right = 0.5cm of l3c4] { };
    \node[node] (l3c6) [right = 0.5cm of l3c5] { };
    % 
    \node[node] (l4c1) [below = 0.1cm of l3c1] { };
    \node[node] (l4c2) [right = 0.5cm of l4c1] { };
    \node[node] (l4c3) [right = 0.5cm of l4c2] { };
    \node[node, thick, blue!70!black] (l4c4) [right = 0.5cm of l4c3] { };
    \node[node] (l4c5) [right = 0.5cm of l4c4] { };
    \node[node] (l4c6) [right = 0.5cm of l4c5] { };
    % 
    \node[node] (l5c1) [below = 0.1cm of l4c1] { };
    \node[node] (l5c2) [right = 0.5cm of l5c1] { };
    \node[node] (l5c3) [right = 0.5cm of l5c2] { };
    \node[node] (l5c4) [right = 0.5cm of l5c3] { };
    \node[node] (l5c5) [right = 0.5cm of l5c4] { };
    \node[node] (l5c6) [right = 0.5cm of l5c5] { };
    % 
    \node[node] (l6c1) [below = 0.1cm of l5c1] { };
    \node[node, thick, red!70!black] (l6c2) [right = 0.5cm of l6c1] { };
    \node[node] (l6c3) [right = 0.5cm of l6c2] { };
    \node[node] (l6c4) [right = 0.5cm of l6c3] { };
    \node[node] (l6c5) [right = 0.5cm of l6c4] { };
    \node[node] (l6c6) [right = 0.5cm of l6c5] { };
    % 
    \node[node] (l7c1) [below = 0.1cm of l6c1] { };
    \node[node] (l7c2) [right = 0.5cm of l7c1] { };
    \node[node] (l7c3) [right = 0.5cm of l7c2] { };
    \node[node] (l7c4) [right = 0.5cm of l7c3] { };
    \node[node] (l7c5) [right = 0.5cm of l7c4] { };
    \node[node] (l7c6) [right = 0.5cm of l7c5] { };
    
    % Axis
    \node (ax) [below left = 0.15cm of l7c1] { };
    \node (ax_y1) [above left = 0.1cm and 0.1cm of l1c1] { };
    \node (ax_y2) [below right = 0.05cm and 0.2cm of l7c6] { };
    
    %
    \draw[->] (ax.center) -- (ax_y1.center);
    \path (ax) -- node [rotate=90,below left=-0.45cm and 1.7cm] {\textbf{Movement Type}} (ax_y1);
    \node (le1) [left = 0.3cm of l1c1] {None};
    \node (le2) [left = 0.3cm of l2c1] {Random};
    \node (le3) [left = 0.3cm of l3c1] {Random 1D};
    \node[thick, blue!70!black] (le4) [left = 0.3cm of l4c1] {Flee};
    \node (le5) [left = 0.3cm of l5c1] {Flee 1D};
    \node[thick, red!70!black] (le6) [left = 0.3cm of l6c1] {Follow};
    \node (le7) [left = 0.3cm of l7c1] {Follow 1D};
    
    %
    \draw[->] (ax.center) -- (ax_y2.center);
    \path (ax) -- node [below right=0.5cm and -1cm] {\textbf{Weapon Type}} (ax_y2);
    \node (ce1) [below = 0.3cm of l7c1] {Barehand};
    \node[thick, red!70!black] (ce2) [below = 0.3cm of l7c2] {Sword};
    \node (ce3) [below = 0.3cm of l7c3] {Bow};
    \node[thick, blue!70!black] (ce4) [below = 0.3cm of l7c4] {Bomb Thrower};
    \node (ce5) [below = 0.3cm of l7c5] {Shield};
    \node (ce6) [below = 0.3cm of l7c6] {Cure Spell};
    
    % 
    \draw[dashed, thick, red!70!black] (le6) -- (l6c2);
    \draw[dashed, thick, red!70!black] (ce2) -- (l6c2);
    
    \draw[dashed, thick, blue!70!black] (le4) -- (l4c4);
    \draw[dashed, thick, blue!70!black] (ce4) -- (l4c4);
    \end{tikzpicture}

    \caption{The map of MAP-Elites population. The red cell represents a melee enemy that follows the player to hit with a sword. The blue cell represents a ranged enemy that flees from the player while throwing bombs towards them.}
    \label{fig:map-representation}
\end{figure}

==> Breno CoG2022/preamble.tex <==
%% Não remover esse arquivo!
%% Alguns pacotes importados alteram o template original
%% Esse arquivo corrige essas alterações

\DeclareCaptionLabelSeparator{dot}{. }
\DeclareCaptionFormat{sbgamestable}{\fontsize{8pt}{8pt}\centering \rmfamily#1\break\scshape#3}
\DeclareCaptionFormat{sbgamessubtable}{\fontsize{8pt}{8pt}\centering\rmfamily#1\scshape#3}
\DeclareCaptionFormat{sbgamesfigure}{\fontsize{8pt}{8pt}\rmfamily#1#2#3}
\captionsetup{labelsep=dot}
\captionsetup[table]{name=TABLE,format=sbgamestable}
\captionsetup[subtable]{name=TABLE,format=sbgamessubtable}
\captionsetup[figure]{format=sbgamesfigure}

\renewcommand{\sectionautorefname}{\uppercase{S}ection}
\renewcommand{\subsectionautorefname}{\uppercase{S}ubsection}
\renewcommand{\figureautorefname}{\uppercase{F}ig.}
\newcommand{\algorithmautorefname}{\uppercase{A}lgorithm}

\usepackage{tikz}
\usetikzlibrary{positioning}

\usepackage{pgfplots, pgfplotstable}
\pgfplotsset{compat=newest}

\pgfplotsset{
    show sum on top/.style={
        /pgfplots/scatter/@post marker code/.append code={%
            \node[
                at={(normalized axis cs:%
                        \pgfkeysvalueof{/data point/x},%
                        \pgfkeysvalueof{/data point/y})%
                },
                anchor=south,
            ]
            {\pgfmathprintnumber{\pgfkeysvalueof{/data point/y}}};
        },
    },
}

\newcommand{\f}{\mkern-2mu f\mkern-3mu}

==> Breno CoG2022/tables/enemy-representation.tex <==
\begin{table*}[!ht]
\centering
\caption{List of attributes of the enemy’s genotype. The line between attributes represents the crossover point. Adapted from \cite{ref:pereira2021procedural}.}
\label{table:enemygenotype}
\small
\begin{tabular}{@{}lccp{8.5cm}@{}}
\toprule
\textbf{Attribute} & \textbf{Type} & \textbf{Range} & \textbf{Details (the attribute defines...)} \\
\midrule
Health & Integer & 1-5 & How many hits an enemy endures. \\
Damage & Integer & 1-4 & How many life points an enemy takes from the player. \\
Attack Speed & Float & 0.75-4.0 & How frequent an enemy shoots a projectile (1/Attack Speed). \\
Movement Type & Nominal & - & How the enemy moves during gameplay. \\
Movement Speed & Float & 0.8-2.8 & How faster the enemy moves. \\
Active Time & Float & 1.5-10.0 & The time in seconds that the enemy moves before resting. \\
Rest Time & Float & 0.3-1.5 & The time in seconds that the enemy rests before moving. \\
\midrule
Weapon Type & Nominal & - & The weapon gameplay properties. \\
Projectile Speed & Float & 1.0-4.0 & How faster the projectile moves towards the player. \\
\bottomrule
\end{tabular}
\end{table*}

==> Breno CoG2022/tables/fitness.tex <==
\begin{table*}[!ht]
% \centering
\caption{Results of fitness obtained after 100 executions of our approach. Each fitness value corresponds to the distance between the input difficulty and the difficulty of the found enemy -- the closer to zero, the better.}
\label{tab:fitness}

    \begin{subtable}[t]{\textwidth}
    \centering
    \caption{Very Easy Difficulty = 11.}
    \label{tab:difficulty11}
    \begin{tabular}{lcccccc}
    \toprule
                  & Barehand   & Sword      & Bow        & Bomb Thrower & Shield     & Cure Spell \\
    \midrule
    None     &  $0.00\pm0.00$ & $0.00\pm0.00$ & $0.01\pm0.01$ & $0.01\pm0.01$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    Random   &  $0.00\pm0.00$ & $0.00\pm0.00$ & $0.01\pm0.01$ & $0.01\pm0.01$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    Random1D &  $0.00\pm0.00$ & $0.00\pm0.00$ & $0.01\pm0.01$ & $0.01\pm0.01$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    Flee     &  $0.00\pm0.00$ & $0.00\pm0.00$ & $0.16\pm0.23$ & $0.21\pm0.38$   & $0.00\pm0.00$ & $0.03\pm0.03$ \\
    Flee1D   &  $0.00\pm0.00$ & $0.00\pm0.00$ & $0.06\pm0.10$ & $0.07\pm0.12$   & $0.00\pm0.00$ & $0.03\pm0.04$ \\
    Follow   &  $0.01\pm0.01$ & $0.01\pm0.01$ & $0.43\pm0.58$ & $0.43\pm0.53$   & $0.01\pm0.02$ & $0.02\pm0.02$ \\
    Follow1D &  $0.00\pm0.00$ & $0.00\pm0.00$ & $0.01\pm0.01$ & $0.01\pm0.01$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    \bottomrule
    \end{tabular}
    \end{subtable}

    \begin{subtable}[t]{\textwidth}
    \centering
    \caption{Easy Difficulty = 13.}
    \label{tab:difficulty13}
    \begin{tabular}{lcccccc}
    \toprule
                  & Barehand   & Sword      & Bow        & Bomb Thrower & Shield     & Cure Spell \\
    \midrule
    None     & $0.00\pm0.01$ & $0.00\pm0.00$ & $0.01\pm0.02$ & $0.01\pm0.02$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    Random   & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.01\pm0.01$ & $0.01\pm0.03$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    Random1D & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.01\pm0.01$ & $0.01\pm0.01$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    Flee     & $0.00\pm0.02$ & $0.00\pm0.01$ & $0.12\pm0.22$ & $0.09\pm0.20$   & $0.00\pm0.01$ & $0.03\pm0.03$ \\
    Flee1D   & $0.00\pm0.01$ & $0.00\pm0.01$ & $0.04\pm0.05$ & $0.04\pm0.05$   & $0.00\pm0.01$ & $0.03\pm0.03$ \\
    Follow   & $0.01\pm0.01$ & $0.01\pm0.01$ & $1.07\pm1.12$ & $1.06\pm0.97$   & $0.01\pm0.01$ & $0.02\pm0.02$ \\
    Follow1D & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.01\pm0.01$ & $0.01\pm0.01$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    \bottomrule
    \end{tabular}
    \end{subtable}

    \begin{subtable}[t]{\textwidth}
    \centering
    \caption{Medium Difficulty = 15.}
    \label{tab:difficulty15}
    \begin{tabular}{lcccccc}
    \toprule
             & Barehand   & Sword      & Bow    & Bomb Thrower  & Shield     & Cure Spell \\
    \midrule
    None     & $0.07\pm0.14$ & $0.06\pm0.14$ & $0.02\pm0.03$ & $0.02\pm0.03$   & $0.08\pm0.18$ & $0.02\pm0.02$ \\
    Random   & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.01$ & $0.00\pm0.01$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    Random1D & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.01$ & $0.00\pm0.01$   & $0.00\pm0.00$ & $0.01\pm0.02$ \\
    Flee     & $0.07\pm0.14$ & $0.08\pm0.23$ & $0.03\pm0.04$ & $0.03\pm0.04$   & $0.08\pm0.22$ & $0.03\pm0.03$ \\
    Flee1D   & $0.05\pm0.11$ & $0.06\pm0.13$ & $0.02\pm0.02$ & $0.02\pm0.03$   & $0.07\pm0.14$ & $0.02\pm0.03$ \\
    Follow   & $0.01\pm0.01$ & $0.01\pm0.01$ & $1.70\pm1.47$ & $2.15\pm1.82$   & $0.01\pm0.01$ & $0.02\pm0.02$ \\
    Follow1D & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.01$ & $0.00\pm0.00$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    \bottomrule
    \end{tabular}
    \end{subtable}

    \begin{subtable}[t]{\textwidth}
    \centering
    \caption{Hard Difficulty = 17.}
    \label{tab:difficulty17}
    \begin{tabular}{lcccccc}
    \toprule
             & Barehand   & Sword      & Bow    & Bomb Thrower  & Shield     & Cure Spell \\
    \midrule
    None     & $1.91\pm0.25$ & $1.90\pm0.20$ & $0.03\pm0.03$ & $0.03\pm0.03$   & $1.91\pm0.21$ & $0.02\pm0.02$ \\
    Random   & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    Random1D & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    Flee     & $1.96\pm0.27$ & $1.94\pm0.27$ & $0.02\pm0.03$ & $0.02\pm0.01$   & $1.96\pm0.27$ & $0.02\pm0.02$ \\
    Flee1D   & $1.98\pm0.27$ & $1.94\pm0.24$ & $0.01\pm0.01$ & $0.01\pm0.01$   & $1.95\pm0.26$ & $0.02\pm0.02$ \\
    Follow   & $0.01\pm0.01$ & $0.01\pm0.01$ & $2.32\pm2.07$ & $2.29\pm2.16$   & $0.01\pm0.01$ & $0.01\pm0.01$ \\
    Follow1D & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    \bottomrule
    \end{tabular}
    \end{subtable}

    \begin{subtable}[t]{\textwidth}
    \centering
    \caption{Very Hard Difficulty = 19.}
    \label{tab:difficulty19}
    \begin{tabular}{lcccccc}
    \toprule
         & Barehand    & Sword       & Bow        & Bomb Thrower & Shield      & Cure Spell \\
    \midrule
    None     & $3.91\pm0.23$ & $3.93\pm0.24$ & $0.04\pm0.04$ & $0.03\pm0.04$   & $3.93\pm0.27$ & $0.02\pm0.02$ \\
    Random   & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    Random1D & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    Flee     & $3.95\pm0.27$ & $3.99\pm0.32$ & $0.02\pm0.02$ & $0.01\pm0.02$   & $3.94\pm0.29$ & $0.02\pm0.02$ \\
    Flee1D   & $3.90\pm0.18$ & $3.89\pm0.17$ & $0.01\pm0.01$ & $0.01\pm0.01$   & $3.91\pm0.18$ & $0.02\pm0.02$ \\
    Follow   & $0.01\pm0.01$ & $0.01\pm0.01$ & $3.14\pm2.39$ & $3.35\pm2.63$   & $0.01\pm0.01$ & $0.01\pm0.01$ \\
    Follow1D & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$   & $0.00\pm0.00$ & $0.01\pm0.01$ \\
    \bottomrule
    \end{tabular}
    \end{subtable}

\end{table*}

==> Breno CoG2022/tables/related-works.tex <==
\begin{table*}[!ht]
\centering
\caption{Enemy generation literature summarizing and comparison with this work. `P' defines the partially generated enemy features.}
\label{table:enemygenerationworks}
\small
\begin{tabular}{@{}p{6cm}cccccc@{}}
\toprule
\textbf{Work} & \textbf{Placement} & \textbf{Amount} & \textbf{Status} & \textbf{Visuals} & \textbf{Adaptive} & \textbf{MAP-Elites} \\
\midrule
Baldwin et al. \cite{ref:baldwin2017mixed} & $\checkmark$ & $\checkmark$ & - & - & - & - \\
Baldwin et al. \cite{ref:baldwin2017towards} & $\checkmark$ & $\checkmark$ & - & - & - & - \\
Liapis \cite{ref:liapis2017multi} & $\checkmark$ & - & - & - & - & - \\
Khalifa et al. \cite{ref:khalifa2018talakat} & $\checkmark$ & $\checkmark$ & P & P & - & $\checkmark$ \\
Pereira et al. \cite{ref:pereira2021procedural} & $\checkmark$ & $\checkmark$ & $\checkmark$ & P & - & - \\
\midrule
Spore \cite{ref:spore} & - & - & P & P & - & - \\
No Man's Sky \cite{ref:nomanssky} & - & - & P & P & - & - \\
Creatures \cite{ref:creatures} & - & - & $\checkmark$ & P & $\checkmark$ & - \\
Diablo 3 \cite{ref:diabloiii} & - & - & P & - & - & - \\
Middle Earth: Shadow of Mordor \cite{ref:shadowofmordor} & - & - & P & - & - & - \\
Left 4 Dead 2 \cite{ref:left4dead2} & $\checkmark$ & $\checkmark$ & - & - & $\checkmark$ & - \\
State of Decay 2 \cite{ref:stateofdecay2} & $\checkmark$ & $\checkmark$ & - & - & $\checkmark$ & - \\
\midrule
This work & $\checkmark$ & - & $\checkmark$ & P & - & $\checkmark$ \\
\bottomrule
\end{tabular}
\end{table*}

==> Breno CoG2022/tables/time.tex <==
\begin{table}[!ht]
\centering
\caption{Results of time in seconds obtained after 100 executions of our approach.}
\label{tab:time}

\begin{tabular}{@{}ccccc@{}}
\toprule
Difficulty & Average & Minimum & Maximum & Standard Deviation \\
\midrule
11         & 0.1608  & 0.1510  & 0.2345  & 0.0126 \\
13         & 0.1609  & 0.1521  & 0.2255  & 0.0115 \\
15         & 0.1597  & 0.1508  & 0.2474  & 0.0145 \\
17         & 0.1621  & 0.1509  & 0.2000  & 0.0106 \\
19         & 0.1581  & 0.1512  & 0.1970  & 0.0072 \\
% 10         & 0.1577  & 0.1506  & 0.1897  & 0.0062 \\
% 18         & 0.1677  & 0.1515  & 0.2369  & 0.0184 \\
% 26         & 0.1586  & 0.1508  & 0.1945  & 0.0068 \\
\bottomrule
\end{tabular}
\end{table}
